Prioritized Generative Replay

Sample-efficient online reinforcement learning often uses replay buffers to store experience for reuse when updating the value function. However, uniform replay is inefficient, since certain classes of transitions can be more relevant to learning. While prioritization of more useful samples is helpful, this strategy can also lead to overfitting, as useful samples are likely to be more rare. In this work, we instead propose a prioritized, parametric version of an agent's memory, using generative models to capture online experience. This paradigm enables (1) densification of past experience, with new generations that benefit from the generative model's generalization capacity and (2) guidance via a family of "relevance functions" that push these generations towards more useful parts of an agent's acquired history. We show this recipe can be instantiated using conditional diffusion models and simple relevance functions such as curiosity- or value-based metrics. Our approach consistently improves performance and sample efficiency in both state- and pixel-based domains. We expose the mechanisms underlying these gains, showing how guidance promotes diversity in our generated transitions and reduces overfitting. We also showcase how our approach can train policies with even higher update-to-data ratios than before, opening up avenues to better scale online RL agents.

==> sections/6_discussion_v1.tex <==
While our framework for conditional generative replay demonstrates strong results, there remain limitations. Firstly, our approach relies on meaningful experience in the agent's memory to densify. In challenging environments where the agent spends a significant amount of time performing unmeaningful behaviors before receiving learning signal, this assumption falls unrealized. 
Secondly, retraining our generative memory periodically \emph{from scratch} represents a significant additional computation burden, especially in the online setting. 
Thirdly, as we show in~\cref{fig:scaling}, \ours cannot yet use much higher synthetic-to-real data ratios. This may simply reflect our use of relatively underpowered diffusion models in \ours, but merits further investigation into the possible ceiling of generative replay.


